Hyperbolic Manifold Regression

Geometric representation learning has recently shown great promise in several machine learning settings, ranging from relational learning to language processing and generative models. In this work, we consider the problem of performing manifold-valued regression onto an hyperbolic space as an intermediate component for a number of relevant machine learning applications. In particular, by formulating the problem of predicting nodes of a tree as a manifold regression task in the hyperbolic space, we propose a novel perspective on two challenging tasks: 1) hierarchical classification via label embeddings and 2) taxonomy extension of hyperbolic representations. To address the regression problem we consider previous methods as well as proposing two novel approaches that are computationally more advantageous: a parametric deep learning model that is informed by the geodesics of the target space and a non-parametric kernel-method for which we also prove excess risk bounds. Our experiments show that the strategy of leveraging the hyperbolic geometry is promising. In particular, in the taxonomy expansion setting, we find that the hyperbolic-based estimators significantly outperform methods performing regression in the ambient Euclidean space.

==> sections/A_diffgeo.tex <==
A Riemannian manifold $(\M, g)$ of dimension $n$ is a topological space $\M$ such that every point $y \in \M$ has a neighbourhood which is homeomorphic to an open set in Euclidean space $\R^n$ and $g$ is a collection of inner product defined in every tangent space $T_{y}\M$ of every point $y \in \M$. Intuitively, the tangent space $T_y \M$ is an approximation of a neighbourhood of $y \in M$ that has a vector space structure. We will denote the inner product of $u, v \in T_y\M$ as $ \langle u, v \rangle_y$. Thanks the inner product structure in every tangent space of the manifold we can compute gradients of functions $f \colon \M \to \R$ that we will denote with $\nabla_{\M} f \colon \mathcal{F}_y (\M) \to T_{y}\M$. Where $F_y(\M)$ is the set of smooth real-valued functions defined on a neighbourhood of $y$.

For any $y_0, y_1 \in \M$ and $v \in T_y\M$ there is a unique smooth \textit{geodesic} curve $\gamma \colon [0,1] \to \M$ such that $\gamma(0) = y_0, \; \gamma(1)=y_1$ and $\frac{d}{dt} \gamma(0) = v$, this curve locally minimizes the path between $y_0$ and $y_1$. Given the geodesic between $y_0$ and $y_1$ with derivative  $\frac{d}{dt} \gamma(0) = v$, the exponential map $Exp_{y_0} \colon T_{y_0}\M \to \M$ maps vector $v \in T_{y_0}\M$ to $y_1$.
A retraction $R_{y} \colon T_y \M \to \M$,  is a first order approximation of the exponential map. Exponential maps are retractions.

\section{Further Experimental Results}
\begin{table}
	\begin{tabular}{lllllll}
	  \toprule
	  & &\multicolumn{5}{c}{Predicted datapoints} \\
	  \cmidrule(r){3-7}
		& & 5             & 10            & 20            & 30            & 50            \\
		\midrule
		\multirow{5}{*}{\bf MR} & Orig     & $2.44\pm0.90$   & $2.12\pm0.36$   & $2.00\pm0.35$   & $2.31\pm0.45$   & $2.21\pm0.36$   \\
		& KRLS     & $46.00\pm56.60$ & $54.10\pm36.10$ & $53.90\pm23.80$ & $66.80\pm25.30$ & $75.80\pm13.30$ \\
		& NN-G     & $23.30\pm44.60$ & $23.10\pm22.00$ & $26.30\pm22.00$ & $24.50\pm10.30$ & $34.70\pm12.30$ \\
		& NN-E     & $45.40\pm57.20$ & $58.60\pm36.00$ & $61.50\pm30.00$ & $68.00\pm17.80$ & $78.60\pm17.40$ \\
		& HSP      & $17.50\pm29.30$ & $22.40\pm22.10$ & $21.80\pm16.50$ & $20.90\pm11.90$ & $26.10\pm9.90$  \\
		\bottomrule
	\end{tabular}
	\caption{Mean rank for WordNet mammals dataset}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../neurips_2019"
%%% End:


==> sections/A_rates.tex <==



In this section prove the result in \cref{thm:rates}. For all required notion related to Riemannian Geometry we refer to the excellent book \cite{lee2003smooth}. The result is the specialization of \cite[Thm. 2 and 4]{Rudi2018}. In particular we recall a key assumption that is required to apply such results. 

\begin{assumption}\label{asm:manifold-regularity}
$\mathcal{M}$ is a complete $n$-dimensional smooth connected Riemannian manifold,
without boundary, with Ricci curvature bounded below and positive injectivity radius.
\end{assumption}

The assumption above imposes basic regularity conditions on the output manifold. A first implication is indeed that. 

\begin{proposition}[Thm. $2$ in \cite{Rudi2018}]\label{prop:geod-smooth}
Let $\manifold{M}$ satisfy \cref{asm:manifold-regularity} and let $\mathcal{Y}\subset\manifold{M}$ is a compact geodesically convex subset of $\manifold{M}$. Then, the squared geodesic distance $d:\manifold{M}\times\manifold{M}\to\R$ is smooth on $\mathcal{Y}$. Moreover, by the proof of Thm.$1$ in the appendix of \cite{Rudi2018}, we have $d^2\in W^{s,2}(\mathcal{Y})$ for any $s>n/2$. 
\end{proposition} 

Leveraging standard results from Riemannian geometry, we can guarantee that the manifolds considered in this paper satisfy the above requirements. For simplicity, we restrict on $\manifold{M}$ corresponding to an open bounded ball in either $\mathcal{P}^n$ or $\Lor^n$. In particular,
\begin{itemize}
\item $\manifold{M}$ has sectional curvature constantly equal to $-1$. Hence the Ricci curvature is bounded from below since we are in a bounded ball in either $\mathcal{P}^n$ or $\Lor^n$. 
\item The injectivity radius is positive (actually lower bounded by $1/(2\cdot 9^{2 + [n/2]})$ with $[n/2]$ the integer parts of $n/2$), see Main Theorem in \cite{martin1989balls}.
\end{itemize}

We see that we are in the hypotheses of \cref{prop:geod-smooth}, from which we conclude the following.

\begin{corollary}\label{cor:geod-smooth}
For any $s\geq 0$, the geodesic distance $d_\Lor$ (respectively $d_{\mathcal{P}}$) belongs to $W^{s,2}(\Y)$ for any compact subspace of $\Lor^n$ (respectively $\mathcal{P}^n$).  
\end{corollary}


This guarantees us that we are in the hypotheses of \cite[Thm. $4$]{Rudi2018}, from which \cref{thm:rates} follows immediately. We note in particular that $d_\Lor^2$ takes the role of the loss function $\bigtriangleup$ in the original theorem. Which needs to be a so-called ``Structure Encoding Loss Function'' (see definition in \cite{Rudi2018}). The latter is guaranteed by \cref{cor:geod-smooth} above. 







